Bandits with many optimal arms

We consider a stochastic bandit problem with a possibly infinite number of arms. We write $p^*$ for the proportion of optimal arms and $\Delta$ for the minimal mean-gap between optimal and sub-optimal arms. We characterize the optimal learning rates both in the cumulative regret setting, and in the best-arm identification setting in terms of the problem parameters $T$ (the budget), $p^*$ and $\Delta$. For the objective of minimizing the cumulative regret, we provide a lower bound of order $\Omega(\log(T)/(p^*\Delta))$ and a UCB-style algorithm with matching upper bound up to a factor of $\log(1/\Delta)$. Our algorithm needs $p^*$ to calibrate its parameters, and we prove that this knowledge is necessary, since adapting to $p^*$ in this setting is impossible. For best-arm identification we also provide a lower bound of order $\Omega(\exp(-cT\Delta^2 p^*))$ on the probability of outputting a sub-optimal arm where $c>0$ is an absolute constant. We also provide an elimination algorithm with an upper bound matching the lower bound up to a factor of order $\log(T)$ in the exponential, and that does not need $p^*$ or $\Delta$ as parameter. Our results apply directly to the three related problems of competing against the $j$-th best arm, identifying an $\epsilon$ good arm, and finding an arm with mean larger than a quantile of a known order.

==> main/lb_unknown_p.tex <==
%\section{Lower bounds, unknown $p^*$}

%\subsection{Cumulative regret}
% \begin{proposition}\label{prop:lbpunkown}



% Consider $\Delta \in [1/4, 3/4]$ and the following two definitions of two reservoir distributions:
% \begin{itemize}
%     \item The reservoir distribution $\Nu_0$ characterised by $p_1 = \frac{1}{2}$ and $p_2 = \frac{1}{2}$ and $\nu_1 = \mathcal B(1/2)$ and $\nu_2 = \mathcal B(1/2 - \Delta)$.
%     \item The reservoir distribution $\Nu_1$ characterised by $p_1 = \frac{1}{2}$ and $p_2 = \frac{1}{2} - \pstar$ and $p_3 = \pstar$ and $\nu_1 = \mathcal B(1/2 )$ and $\nu_2 = \mathcal B(1/2 - \Delta)$ and $\nu_3 = \mathcal B(1/2 + \Delta)$.
% \end{itemize}
% Let $A>1$. If $\pstar \lesssim 1/(A\log(T))$, an algorithm achieves the bound $\E_{\Nu_0}\left[R(T)\right] > A\frac{\log(T)}{\Delta}$ then it must be that $\E_{\Nu_1}\left[R(T)\right] > T\Delta$.% for $\pstar$ approx $\frac{1}{\log(T)}$
% \end{proposition}
% \begin{proof}
% Let $\tilde \mu = (\tilde \mu_j)_{j \leq T}$ be $T$ i.i.d.~means corresponding to $T$ i.i.d.~distributions sampled according to the reservoir distribution $\Nu_1$. Note that $\tilde \mu_j \in \{1/2-\Delta, 1/2, 1/2+\Delta\}$. Write also $\tilde \mu' = (\tilde \mu_j')_{j \leq T}$ for the vector of means such that $\tilde \mu_j' = \tilde \mu_j$ if $\tilde \mu_j' \in\{1/2-\Delta, 1/2\}$, and $\tilde \mu_j' = 1/2 - \Delta$ otherwise. 

% \begin{align*}
%     \KL(\mathbb E_{\Nu_1} \mathbb P_{\tilde \mu'}^{\mathfrak A}, \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}) &\leq \mathbb E_{\Nu_1} \Bigg[\KL(\mathbb P_{\tilde \mu'}^{\mathfrak A}, \mathbb P_{\tilde \mu}^{\mathfrak A})\Bigg] = \mathbb E_{\Nu_1} \Bigg[\sum_{j \leq T} \mathbb E_{\tilde \mu', \mathfrak A}[T_j] \kl(\tilde \mu_j', \tilde \mu_j)\Bigg]\\
%     &\leq  \mathbb E_{\Nu_1} \Bigg[\sum_{j \leq T} \mathbb E_{\tilde \mu', \mathfrak A}[T_j] \frac{\Delta^2}{16} \mathbf 1\{\tilde \mu_j = 1/2+\Delta\} \Bigg]\\
%     &=  \mathbb E_{\Nu_0} \Bigg[\sum_{j \leq T} \mathbb E_{\tilde \mu', \mathfrak A}[T_j] \frac{\Delta^2}{16} \mathbf 1\{\tilde \mu_j' = 1/2-\Delta\} 2\pstar \Bigg],\\
%     &= \frac{\pstar\Delta}{8} E_{\Nu_0} \left[ R(T)\right]
% \end{align*}


% before continuing we recall the following Lemma, see Lemma 3 \cite{hadiji2019polynomial}.
% \begin{lemma}
% Let $\P$ and $\Q$ be probability measures, for any random variable $Z \in [0,1]$,
% \[|\E_{\P}[Z] - \E_{\Q}[Z] | \leq \sqrt{\frac{\KL\left(\P,\Q\right)}{2}}\]\;.
% \end{lemma}
% The proof of Proposition \ref{prop:lbpunkown} now proceeds as follows,
% \begin{align*}
% \E_{\Nu_1}\P_{\tilde \mu}^{\mathfrak A} \left[ R(T) \right] &= T\Delta\left(1-\E_{\Nu_1} \left[\frac{\sum_{j \leq T} \mathbb E_{\tilde \mu, \mathfrak A}[T_j] \mathbf 1\{\tilde \mu_j = 1/2+\Delta\}}{T}\right]\right)\\
% &\geq T\Delta\left(1-\frac{1}{T}\E_{\Nu_1} \left[\sum_{j \leq T} \mathbb E_{\tilde \mu, \mathfrak A}[T_j] \mathbf 1\{\tilde \mu_j = 1/2+\Delta\}\right] - \sqrt{\frac{\Delta \pstar \E_{\Nu_0} \left[ R(T)\right]}{48}}\right)\\
% &\geq T\Delta\left(1-\frac{1}{T\Delta}\E_{\Nu_1}\P_{\tilde \mu'}^{\mathfrak A} \left[R(T)\right] - \sqrt{\frac{\Delta \pstar \E_{\Nu_0} \left[ R(T)\right]}{48}}\right)
% \end{align*}
% Hence if we assume $E_{\Nu_0} \left[ R(T)\right] \leq \frac{2}{\Delta}$ we have, 

% $$\E_{\Nu_1}\P_{\tilde \mu'}^{\mathfrak A} \left[R(T)\right] \vee \E_{\Nu_1}\P_{\tilde \mu}^{\mathfrak A} \left[R(T)\right] \geq cT\Delta$$




%\begin{theorem}\label{thm:unkownpcumulative}
%Let $\pstar \leq \frac{1}{4}$ and $c>0$ such that $T \geq \left(\frac{c\log(T)}{\pstar\Delta^2}\right)^2$, for any bandit algorithm $\mathfrak A$ such that,

%$$\max_{B \in \mathfrak B_{\Delta,\pstar}} R^{\mathfrak A}_{F}(T) \leq \frac{c\log(T)}{\pstar\Delta}\;,$$ 

% \al{In the proof you use the regret in the smallest model corresponding to $\pstar$ (in which $
% \Nu_0$ is), namely you would require instead of what you have
% $$\max_{B \in \mathfrak B_{\Delta,\pstar}} R^{\mathfrak A}_{F}(T) \leq c \frac{\log(T)}{\pstar\Delta}\;,$$ 
% where $c>0$ is an arbitrarily large constant - it is important to introduce $c$ as you want to make sure that you are larger than the minimax rate in model $\pstar$ here... But in fact this is truly what you need and it goes nicely through in the proof - you will require $c \lesssim \pstar/\qstar$, which makes perfect sense!
% }
%one has that,

% \[\forall \pstar \leq \frac{\qstar}{c}, \exists F \in \mathfrak B_{\Delta,p} : R^{\mathfrak A}_{F}(T) \geq \sqrt{T}\Delta\;.\]

%\[\forall \qstar \leq \frac{c\pstar}{4}, \exists F \in \mathfrak B_{\Delta,\qstar} : R^{\mathfrak A}_{F}(T) \geq \sqrt{T}\Delta \;.\]

%\end{theorem}
%\begin{proof}[Proof of Theorem~\ref{thm:unkownpcumulative}]

%We consider a similar setting to that in the proof of Theorem~\ref{thm:LBsimple} although with a slightly different construction of $\Nu_0, \Nu_1$.
%Consider $\Delta \in (0, 1/4)$ and the following two definitions of two reservoir distributions:
%\begin{itemize}
%    \item The reservoir distribution $\Nu_0$ characterised by $p_1 = \pstar$ and $p_2 = 1-\pstar$ and $\nu_1 = \mathcal B(1/2)$ and $\nu_2 = \mathcal B(1/2 - \Delta)$.
%    \item The reservoir distribution $\Nu_1$ characterised by  $p_1 = \qstar$, $p_2 = \pstar$ and $p_3 = 1- \qstar - \pstar$ and $\nu_1 = \mathcal B(1/2 +\Delta)$ and $\nu_2 = \mathcal B(1/2 )$ and $\nu_3 = \mathcal B(1/2 - \Delta)$.
%\end{itemize}

%We define $\tilde \mu, \tilde \mu'$, and associated expectations and probabilities as in the proof of Theorem \ref{thm:LBsimple}. Assume $E_{\Nu_0} \left[ R(T)\right] \leq \frac{\log(T)}{\qstar\Delta}$, otherwise the result is immediate. Now, following the same procedure as therein we obtain also for these priors Equation~\eqref{eq:KLineq}:
%\begin{align*}
%    \KL(\mathbb E_{\Nu_0} \mathbb P_{\tilde \mu'}^{\mathcal A}, \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathcal A}) &= \KL(\mathbb E_{\Nu_1} \mathbb P_{\tilde \mu'}^{\mathfrak A}, \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}) \nonumber\\
%    &\leq \mathbb E_{\Nu_1} \Bigg[\KL(\mathbb P_{\tilde \mu'}^{\mathfrak A}, \mathbb P_{\tilde \mu}^{\mathfrak A})\Bigg] = \mathbb E_{\Nu_1} \Bigg[\sum_{j \leq T} \mathbb E_{\tilde \mu'}^{ \mathfrak A}[T_j] \kl(\tilde \mu_j', \tilde \mu_j)\Bigg] \nonumber\\
%    &\leq  \mathbb E_{\Nu_1} \Bigg[\sum_{j \leq T} \mathbb E_{\tilde \mu'}^{\mathfrak A}[T_j] \frac{\Delta^2}{16} \mathbf 1\{\tilde \mu_j = 1/2+\Delta\} \Bigg] \nonumber\\
%    &=  \mathbb E_{\Nu_0} \Bigg[\sum_{j \leq T} \mathbb E_{\tilde \mu', \mathfrak A}[T_j] \frac{\Delta^2}{16} \mathbf 1\{\tilde \mu_j' = 1/2-\Delta\} \frac{\qstar}{1 - \pstar} \Bigg],\\
%    &= \frac{\qstar\Delta}{8} E_{\Nu_0} \left[ R(T)\right] \leq \frac{c\qstar}{8\pstar}\log(T), \leq \frac{1}{2}\log(T)
%\end{align*}
% \al{There with the assumption in red you would get
% $$\frac{c\qstar\log T}{\pstar},$$
% which is quite nice as $\qstar/\pstar<1$... This allows you to loosen $c$ here - you just need $c \lesssim \pstar/\qstar$ to have the $\log T/2$ bound.

% }

%since by definition of $\Nu_0, \Nu_1$, conditionally on $\tilde \mu_j' = 1/2-\Delta$, the probability that $\tilde \mu_j = 1/2+\Delta$ is $\frac{\qstar}{1 - \pstar} \leq 2\qstar$, and otherwise it is $0$. And where the final inequality comes from our assumption $\pstar > \frac{c\qstar}{4}$.

%\begin{align*}
%    \mathbb E_{\Nu_0} \mathbb P_{\tilde \mu}^{\mathfrak A}(E) + \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu'}^{\mathfrak A}(E^C) &\geq \frac{1}{2} \exp\Bigg(-\KL(\mathbb E_{\Nu_1} \mathbb P_{\tilde \mu'}^{\mathfrak A}, \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A})\Bigg)\;,\\
%    &\geq \frac{1}{2\sqrt{T}}\;.
%\end{align*}
%Now consider the event, 

%\[E := \Bigg\{\sum_{j \leq T} T_j  \mathbf 1\{\tilde \mu_j' = 1/2\}> T/2 %\frac{\log(T)\sqrt{T}}{\pstar \Delta^2}
%\Bigg\}\;.\]

%From our assumption upon $\mathfrak{A}$ we have that under reservoir distribution $\Nu_0$, 
%\[\mathbb E_{\Nu_0} \mathbb P_{\tilde \mu'}^{\mathfrak A}(E) \leq \frac{\log(T)}{\qstar T\Delta^2}\;.\]

%thus,

%\[\mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}(E^C) \geq \frac{1}{2\sqrt{T}} - \frac{\log(T)}{\qstar T\Delta^2} \geq \frac{1}{4\sqrt{T}}\]
%where the final line comes from our assumption on $\pstar, T$ and $c$.

%\end{proof}

% For $k \in [K] \backslash 1$ we define the following sequence of environments,
% \[
% \nu_l^k=
%     \begin{cases}
%       \cB(1/2 + \Delta) & \text{if}\ l = k \\
%       \cB(1/2) & \text{if}\;l=1
%       \\\cB(1/2 - \Delta) & \text{if}\;k\; \mathbf{otherwise}
%     \end{cases}\,.
% \]
% where, $p_l^k = \frac{1}{K}$ for all $l,K \in [K]$
% furthermore we define the environment $\nu_1$ as,

% \[
% \nu_l^1=
%     \begin{cases}
%       \cB(1/2, \sigma^2) & \text{if}\;l=1
%       \\\cB(1/2 - \Delta, \sigma^2) & \text{otherwise}
%     \end{cases}
% \]
% with 
% \[
% p_l^1=
%     \begin{cases}
%       \frac{1}{2} & \text{if}\;l=1
%       \\\frac{1}{2(K-1)} &\text{otherwise}
%     \end{cases}
% \]

% We first construct the Canonical bandit model, see \cite{hadiji2019polynomial}. For all $t\in[T]$ we define the measurable space $\left(\Omega_t,\cF_t\right)$ with  $\Omega_t = \prod_{i\in[t]}(\cA \times \R)$ and $\cF_t = \mathfrak{B}(\Omega_t)$.  A strategy of the leaner is a sequence of probability kernels $\left(\pi_t\right)_{[T]}$ where at time $t$, $\pi_t$ maps from $\Omega_{t-1}$ to $\cA$, modelling the choice of arm at time $t$. 
% For each environment $i$ and time $t$ we also define a probability kernel $L_t$, mapping from $\Omega_t \times \cA$ to $\R$, which models the reward, explicitly for all $B\in \mathfrak{B}(\R)$,

% $$L_{i,t}(a_1,y_1,...,a_t,y_t,B) = \sqrt{\frac{1}{\pi}}\int_B \exp\left(\frac{-(x - \mu_{i,a_t})^2}{2}\right).$$ 

% We can now define the probability measure $\P_{i,t}$ on $(\Omega_t,\cF_t)$ as  $\P_{i,t}= L_{i,t}(\pi_t \P_{i,t})$. Let $\E_{i}$ denote expectation with respect to $\P_{i,T}$. 

% Double application of the chain rule for $\kl$-divergence, see \cite[p.~21]{hadiji2019polynomial} for details, leads to the following proposition, 
% \begin{proposition}\label{prop:kl}
% \[\kl\left(\P_{0,T},\P_{i,T}\right) = \E_0\left[\sum_{i\in[K]}\kl\left(\cN(\mu_{0,a_t},1),\cN\left(\mu_{i,a_t},1)\right)\right)\right]\]
% \end{proposition}

% Let $T_i$ be the number of times a learner samples arm $i$. It follows directly from Proposition \ref{prop:kl} that,
% \begin{equation}
%     \kl\left(\P_0,\P_i\right) = 2\Delta^2\E_0\left[T_i\right]
% \end{equation}

% before continuing we recall the following Lemma, see Lemma 3 \cite{hadiji2019polynomial}.
% \begin{lemma}
% Let $\P$ and $\Q$ be probability measures, for any random variable $Z \in [0,1]$,
% \[|\E_{\P}[Z] - \E_{\Q}[Z] | \leq \sqrt{\frac{\kl\left(\P,\Q\right)}{2}}\]\;.
% \end{lemma}
% The proof of Proposition \ref{prop:lbpunkown} now proceeds as follows,
% \begin{align*}
% \frac{1}{K}\sum_{[K]} R_i &= T\Delta\left(1-\frac{1}{K}\sum_{[K]}\E_{i}\left[\frac{T_i}{T}\right]\right)\\
% &\geq T\Delta\left(1-\frac{1}{TK}\sum_{[K]}\E_{1}[T_i] - \sqrt{\frac{\Delta^2\sum_{[K]}\E_1[T_i]}{K}}\right)\\
% &\geq T\Delta\left(1-\frac{1}{K} - \sqrt{\frac{\Delta R_1}{K}}\right)
% \end{align*}
% Hence if we assume $R_0 \leq \frac{2}{\Delta}$ we have, 

% $$\frac{2}{K}\sum_{even} R_i \geq cT\Delta$$

% \end{proof}

% \subsection{Simple regret}

% \begin{theorem}\label{unkownpsimple}
% Let $\qstar>0$, for any bandit algorithm $\mathfrak A$ such that,


% $$\max_{B \in \mathfrak B_{\Delta,\qstar}} e^{\mathfrak A}_{B}(T) \leq \exp\left(-T \qstar \Delta^2\right)$$
% \al{In fact this assumption is not so realistic I think as this is smaller than the minimax lower bound over the class $q^*$ - you should assume $E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}(E) \leq \exp\left(-cT\qstar\Delta^2 \right)$ where $c>0$ is an arbitrarily small universal constant.}

% one has that,

% \[\forall \pstar > \qstar, \exists F \in \mathfrak B_{\Delta,\pstar} : e^{\mathfrak A}_{F}(T) \geq \exp\left(-T \qstar \Delta^2\right)\;.\]

% \end{theorem}

% \begin{proof}
% We consider a similar setting to that in the proof of Theorem~\ref{thm:LBsimple} although with a slightly different construction of $\Nu_0, \Nu_1$.
% Consider $\Delta \in (0, 1/4)$ and the following two definitions of two reservoir distributions:

% \begin{itemize}
%     \item The reservoir distribution $\Nu_0$ characterised by $p_1 = \pstar$ and $p_2 = 1- \pstar$ and $\nu_1 = \mathcal B(1/2)$ and $\nu_2 = \mathcal B(1/2 - \Delta)$.
%     \item The reservoir distribution $\Nu_1$ characterised by $p_1 = \pstar$ and $p_2 = 1 - \pstar - \qstar$ and $p_3 = \qstar$ and $\nu_1 = \mathcal B(1/2 )$ and $\nu_2 = \mathcal B(1/2 - \Delta)$ and $\nu_3 = \mathcal B(1/2 + \Delta)$.
% \end{itemize}

% We define $\tilde \mu, \tilde \mu'$, and associated expectations and probabilities as in the proof of Theorem \ref{thm:LBsimple}. Now, following the same procedure as therein we obtain also for these priors Equation~\eqref{eq:KLineq}:
% \begin{align*}
% \KL(\mathbb E_{\Nu_0} \mathbb P_{\tilde \mu'}^{\mathfrak A}, \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}) &\leq  \mathbb E_{\Nu_0} \Bigg[\sum_{j \leq T} \mathbb E_{\tilde \mu', \mathfrak A}[T_j] \frac{\Delta^2}{16} \mathbf 1\{\tilde \mu_j' = 1/2-\Delta\} \frac{\qstar}{1 - \pstar} \Bigg],\\
% &\leq  \frac{T\qstar\Delta^2}{8}   
% \end{align*}

% Let us write $\hat a(T)$ for the arm that the algorithm $\mathfrak A$ recommends. Set 
% $$E = \{\tilde \mu_{\hat a(T)} = 1/2\}.$$

% Now applying Pinskers inequality,
% \begin{align*}
%     \mathbb E_{\Nu_0} \mathbb P_{\tilde \mu'}^{\mathfrak A}(E^C) + \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}(E) &\geq \frac{1}{2} \exp\Bigg(-\KL(\mathbb E_{\Nu_0} \mathbb P_{\tilde \mu'}^{\mathfrak A}, \mathbb E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A})\Bigg)\;,\\
%     &\geq \exp\left(-\frac{T\qstar\Delta^2}{8} \right)\;.
% \end{align*}
% Note that via our assumption on $\mathfrak A$ we have that $E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}(E) \leq \exp\left(-T\qstar\Delta^2 \right)$ \al{In fact this assumption is not so realistic I think as this is smaller than the minimax lower bound over the class $q^*$ - you should assume $E_{\Nu_1} \mathbb P_{\tilde \mu}^{\mathfrak A}(E) \leq \exp\left(-cT\qstar\Delta^2 \right)$ where $c>0$ is an arbitrarily small universal constant.}, thus,

% \[E_{\Nu_0} \mathbb P_{\tilde \mu}^{\mathfrak A}(E^C) \geq \exp\left(-\frac{T\qstar\Delta^2}{4} \right)\]

% \end{proof}

